On the Runtime-Efficacy Trade-off of Anomaly Detection Techniques for Real-Time Streaming Data

Ever growing volume and velocity of data coupled with decreasing attention span of end users underscore the critical need for real-time analytics. In this regard, anomaly detection plays a key role as an application as well as a means to verify data fidelity. Although the subject of anomaly detection has been researched for over 100 years in a multitude of disciplines such as, but not limited to, astronomy, statistics, manufacturing, econometrics, marketing, most of the existing techniques cannot be used as is on real-time data streams. Further, the lack of characterization of performance -- both with respect to real-timeliness and accuracy -- on production data sets makes model selection very challenging. To this end, we present an in-depth analysis, geared towards real-time streaming data, of anomaly detection techniques. Given the requirements with respect to real-timeliness and accuracy, the analysis presented in this paper should serve as a guide for selection of the "best" anomaly detection technique. To the best of our knowledge, this is the first characterization of anomaly detection techniques proposed in very diverse set of fields, using production data sets corresponding to a wide set of application domains.

==> Bio.tex <==
\section{Biography}


==> Related.tex <==
\section{Related Work} \label{sec:rel}

\input surveys


==> accspeedfigs.tex <==
\begin{figure*}[!t]
\centering
    \begin{subfigure}[t]{0.33\textwidth}
        \raisebox{-\height}{\includegraphics[width=\textwidth]{robustness}}
        \caption{Illustration of the impact of lack of robustness}
        \vspace*{-2mm}
        \label{fig:robustness}
    \end{subfigure}
    \hfill
    \hspace*{-4mm}
    \begin{subfigure}[t]{0.33\textwidth}
        \raisebox{-\height}{\includegraphics[width=\textwidth]{tdigest_hysterisis}}
        \caption{Peformance of {\em t-digest} anomaly bursts}
        \vspace*{-2mm}
        \label{fig:tdigest_hysterisis}
    \end{subfigure}
    \hfill
    \hspace*{-4mm}
    \begin{subfigure}[t]{0.33\textwidth}
        \raisebox{-\height}{\includegraphics[width=\textwidth]{hotsax_similar_anomaly}}
        \caption{HOTSAX similar anomalies}
        \vspace*{-2mm}
        \label{fig:hotsax_anomaly}
    \end{subfigure}
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%second row
    \begin{subfigure}[t]{0.33\textwidth}
        \raisebox{-\height}{\includegraphics[width=\textwidth]{iforest_robustness}}
        \caption{Anomaly Score Separation}
        \vspace*{-2mm}
        \label{fig:anom_score}
    \end{subfigure}
    \hfill
    \hspace*{-4mm}
    \begin{subfigure}[t]{0.33\textwidth}
        \raisebox{-\height}{\includegraphics[width=\textwidth]{rpca_sparse}}
        \caption{Illustration of the performance of RPCA Sparse Component in the presence
                 of trend}
        \vspace*{-2mm}
        \label{fig:rpca_trend}
    \end{subfigure}
    \hfill
    \hspace*{-4mm}
    \begin{subfigure}[t]{0.33\textwidth}
        \raisebox{-\height}{\includegraphics[width=\textwidth]{hotsax_dbstream}}
        \caption{HOTSAX and DBStream for {\em health-qtdb/0606}}
        \vspace*{-2mm}
        \label{fig:hotsax_dbstream}
    \end{subfigure}
\vspace*{-2mm}
\caption{Accuracy Analysis}
%\vspace*{-6mm}
\label{fig:accanalysis}
\end{figure*}





\iffalse

\begin{figure}[!h]
\centering
\includegraphics[width=\linewidth, height=3in]{robustness}
\vspace*{-4mm}
\caption{Illustration of the impact of lack of robustness}
\vspace*{-2mm}
\label{fig:robustness}
\end{figure}

\begin{figure}[!h]
\centering
\includegraphics[width=\linewidth, height=3in]{tdigest_hysterisis}
\vspace*{-4mm}
\caption{Peformance of {\em t-digest} anomaly bursts}
\vspace*{-2mm}
\label{fig:tdigest_hysterisis}
\end{figure}

\begin{figure}[!h]
\centering
\includegraphics[width=\linewidth, height=3in]{hotsax_similar_anomaly}
\vspace*{-4mm}
\caption{HOTSAX similar anomalies}
\vspace*{-2mm}
\label{fig:hotsax_anomaly}
\end{figure}

\begin{figure}[!h]
\centering
\includegraphics[width=\linewidth, height=3in]{iforest_robustness}
\vspace*{-4mm}
\caption{Anomaly Score Separation}
\vspace*{-2mm}
\label{fig:anom_score}
\end{figure}

\begin{figure}[!h]
\centering
\includegraphics[width=\linewidth, height=3in]{rpca_sparse}
\vspace*{-4mm}
\caption{Illustration of the performance of RPCA Sparse Component in the presence
         of trend}
\vspace*{-2mm}
\label{fig:rpca_trend}
\end{figure}

\begin{figure}[!h]
\centering
\includegraphics[width=\linewidth, height=3in]{hotsax_dbstream}
\vspace*{-4mm}
\caption{HOTSAX and DBStream for {\em health-qtdb/0606}}
\vspace*{-2mm}
\label{fig:hotsax_dbstream}
\end{figure}

\fi


==> robust.tex <==
A useful way to understand robustness is to think in terms of the Influence Function which describes the effect of changing a
given point $y$, on a functional estimator $T(F)$ for an assumed underlying distribution $F$. $T$ here can be a statistical estimate like
location or scatter. $F$ is an assumed distribution like Normal or Poisson. Mathematically the influence function is the first derivate
of T at an underlying distribution F.
\begin{equation}
IF(y;T,F) =  \lim_{t \to 0} \frac{T((1-t)F + t\Delta_{y}) - T(F)}{t}
\end{equation}
One can use the $IF$ to understand the behavior of an estimator in the presence of extreme outliers. For eg. if T is the arithmetic mean,
a change in a single value can make the $IF$ unbounded. So the mean is not resistant to any outliers. To quantify the maximum bias caused by
contamination of $F$ we use the supremum norm over $y$, called the gross error sensitivity
\begin{equation}
\gamma* = \sup_{y} |IF(y;T,F)|
\end{equation}
Estimate that have finite $\gamma*$ are said to be B-robust (bias). The $L_{2}$ norm of the $IF$ gives us the asymptotic variance of the estimator.
\begin{equation}
V(T,F) = \int IF(y;T,F)^2 dF
\end{equation}
$V(T, F)$ is a measure of the tightness of the confidence interval around the estimator $T$, and is hence inversely proportional to the efficiency
of $T$. $\gamma*$ and $V(T,F)$ cannot be improved simultaneously, and all estimators improve one at the expense of the other. Estimators that
achieve the best efficiency for a given finite upper bound of $\gamma*$, are called optimally B-robust. While the IF measures local robustness to
infinitesimal changes, global robustness is quantified by the Breakdown Point ($BDP$), defined as the maximum number of outliers to which the
statistic can remain resistant. As we saw with the mean a single point can make it unbounded, so its $BDP$ is 0. Best achievable $BDP$
is $1/2$. In practice, the most important concepts are error sensitivity and breakdown point. With the large sample sizes, the impact of efficiency loss
can be compensated by larger samples, given the variance is constant. We now analyze some of the important robust estimators.

\noindent \\
{\bf M-estimators} \\
Given a sample $Y={(y_1, y_2, ... y_n)}$, M-estimators are estimators that solve the equations
\begin{equation}
min \sum_{i=1}^{n} \rho(y_{i}, T_{n})
\qquad
\sum_{i=1}^{n} \psi(y_{i}, T_{n}) = 0
\end{equation}
where $\psi = \frac{\partial \rho}{\partial T}$.
For the maximum likelihood estimator $\rho=-\ln f_T(y)$, so M-estimators are a generalized form of MLE.

For a single dimension, Huber M-estimator\cite{huber1964_mest} (also called the minmax estimator) is the optimal B-robust location estimator for the normal model $\Phi$, given by
\begin{equation}
\psi_{b}(y) = min\{b, max\{y, -b\}\}
\end{equation}
For scatter estimation, the Median Absolute Deviation (MAD) is a B-robust estimator with asymptotic efficiency of $36.7\%(\Phi)$.
Both MAD and Huber minmax have maximal $BDP$ of $0.5$. MAD is defined as the median of the absolute deviations from the median($\widetilde{m}$).
\begin{equation}
MAD = med\{y_i-med_j\{y_j\} \}
\end{equation}
Most location estimators are sensitive to scatter, and MAD is a computationally non-intensive scatter estimate for standardization.

\noindent \\
{\bf L-estimators} \\
L-estimators are computationally less expensive but relatively inefficient alternatives to M-estimators as they do not need to solve a convex optimization problem. They
are defined as weighted sums of ordered variables.
\begin{equation}
T(Y) = \sum_{1}^{n} a_i*y_{:i}
\end{equation}
where $a_i$ is the weight and $y_{:i}$ is an ordered value.
The Median($\widetilde{m}$) is an L-estimator for location where only the weights for the central data point are non-zero. Median has minimal error sensitivity
and maximal $BDP$, but it suffers from low asymptotic efficiency of $63.7\%(\Phi)$.
Inter-Quartile Range(IQR) \cite{adjboxplot_hubert_2004} is an L-estimator for scatter with a low gross error sensitivity and asymptotic efficiency of $36.7\%(\Phi)$.
Its $BDP$ is significantly worse($0.25$), because IQR can suffer from contamination just from one side.

\noindent \\
{\bf W-estimators} \\
W-estimators are weighted estimators, given by
\begin{equation}
T(Y) = \frac{\sum_{1}^{n} w_i*y_i}{\sum_{1}^{n}w_i}
\end{equation}
where $w_i$ is itself dependent on $T$, $w_i = w(y_i-T)$
Thus one can solve for $T$ using Iteratively Re-weighted least squares which is well known for solving Logistic Regression problems.
Popular weights are Tukey's biweight\cite{tukey_biweight_1974} and Huber weight\cite{huber_robust_1981}.

\noindent \\
{\bf Redescending M-estimators} \\
These are a special class of M-estimators which are able to completely reject very extreme values. They achieve this by zeroing out the $\psi$
function outside a certain range. Notable examples are Hampel's 3-part redescending estimator and Tukey's Biweight estimator.\cite{tukey_biweight_1974}.
These estimators are computationally more expensive than Huber estimator, but offer slightly improved efficiency. This is understandable because
they complete reject extreme outliers, but down weight moderate outliers, whereas Huber's minmax estimator treats all outliers similarly. Redescending
M-estimators can be as much as $20\%$ more efficient than M-estimators for heavy tailed distributions like the Cauchy Distribution.

\noindent \\
{\bf Scale estimators ($Q_n$, $S_n$ and $\tau$)} \\
Until now we have discussed a number of optimally robust location estimators, but our best scatter estimator MAD is not optimally B-robust
because of its low asymptotic efficiency. $Q_n$ estimator\cite{rousseeuw_alternatives_1993} has a higher efficiency that MAD with similar robustness
properties. $Q_n$ can be also be applied for asymmetric distributions (e.g. Exponential) for which MAD does not capture the scatter appropriately.
Finally $\tau$ estimator\cite{yohai_tau_estimator} is a scale estimator with a $BDP$ of 0.5, has high robustness, and is highly efficient at the normal model.
$\tau$ is an M-estimator where the $\psi$ function is a weighted average of two different $psi$ functions,
\begin{equation}
\psi_{\tau} = W_0*\psi_1 +\psi_2
\end{equation}
$\psi_1$ a very robust estimate and $\psi_2$ a very efficient estimate. The weights adapt according to the underlying errors. Under the normal model,
$\tau$ has a $BDP$ of $0.5$ and efficiency of $95\%$.

\noindent \\
{\bf Student's $t$-distribution} \\
$t$-distribution\cite{students_t} is often used as an alternative to the normal model in the presence of heavy tails in the data. The three parameters
of interest are mean($\mu$), deviation($\sigma$) and degrees of freedom($\nu$). It can be shown that these parameters can be estimated by
M-estimators of the following form -
\begin{equation}
\begin{split}
\psi_{\mu} (y) = \frac{(\nu + 1)y}{y^2 + \sigma^2\nu} \qquad
\end{split}
\begin{split}
\psi_{\sigma} (y) = \frac{\nu}{\sigma}.\frac{(\sigma^2 - y^2)}{\nu\sigma^2 + y^2}
\end{split}
\end{equation}
where $\psi_{\mu}$, $\psi_{\sigma}$ are robust estimators as long as $\nu$ is not estimated from the data as well\cite{student_mest}. $\nu$ is usually
set to a lower value (5-10) or estimated proportional to the sample size.
The Generalized Extreme Studentized Deviate (ESD) test \cite{rosner_percentage_1983} uses the $t$-distributiuon to detect outliers in a sample,
by performing iterative hypothesis tests. It requires an upper bound on the number of anomalies ($a$), which helps control the false
alarm rate effectively(CFAR). ESD computes this test statistic for the `$a$` most extreme values,
\begin{equation}
T_a = \frac{max_a |y-\mu|}{\sigma}
\end{equation}
This statistic is then compared to a critical value defined by $\lambda_a$,
\begin{equation}
\lambda_a = \frac{(n-a)t_{p,n-a-1}}{\sqrt{(n-a+1+t_{p,n-a-1})(n-a+1)}}
\end{equation}
where $p$ stands for the statistical significance and $(n-a-1)$ is the degree of freedom in $t_{p,n-a-1}$.
If $T_a$ exceeds $\lambda_a$, the value is tagged as anomalous and removed
from the sample. $\lambda_a$ is recalculated for the next iteration. Even if no anomalous observations are found, ESD continues until the test has run for
$a$ outliers.


==> surveys.tex <==
%\subsection{AD Surveys} \label{sec:survey}

There have been over 1000 different works on anomaly detection, and thus there
have been a number of commendable approaches that have tried to organize and
compare these works. Chandola et al.\cite{chandola_anomaly_2009} came out with
a seminal survey on various AD techniques organized by research domains(e.g.
Statistics, Clustering) as well as application domains(e.g. Process Control,
Network Intrusion).  Gupta et al\cite{aggarwal_outlier_temporal,
aggarwal_outlier_2013} came out with an organization for outlier detection for
temporal data.  They analyzed techniques for time series, data streams,
distributed data streams, spatio-temporal streams and network data. They
present an exhaustive discussion on the various AD formulations and techniques
for temporal data. Previous works by Hodge et al.\cite{hodge_survey_2004}
covered techniques in diverse domains like medical imaging, computer vision,
fault diagnosis and pharmaceutical research.

  There has also been work surveying AD for specific domains. Gogoi et
al.\cite{gogoi_survey_2011} and Bhuyan et al.\cite{bhuyan_survey_2012} outline
various incremental techniques for network anomaly detection. Barnette et
al.\cite{barnett_outliers_1994} dedicate a full book for understanding outliers
in statistical data. Ndong et al\cite{ndong_signal_2011} compare various AD
techniques from signal processing domain.  Chin et al.\cite{chin_symbolic_2005}
provide a comparative analysis of symbolic representations in time series.
Zhange et al.\cite{zhang_survey_wsn_2010} provide a survey of techniques used
in wireless sensor networks.

  Most of these surveys provide a great landscape for the research directions
in AD, but do not delve into enough nuance to serve as a guide for model
selection and comparison.

